AutoVP: An Automated Visual Prompting Framework and Benchmark

Visual prompting (VP) is an emerging parameter-efficient fine-tuning approach to adapting pre-trained vision models to solve various downstream image-classification tasks. However, there has hitherto been little systematic study of the design space of VP and no clear benchmark for evaluating its performance. To bridge this gap, we propose AutoVP, an end-to-end expandable framework for automating VP design choices, along with 12 downstream image-classification tasks that can serve as a holistic VP-performance benchmark. Our design space covers 1) the joint optimization of the prompts; 2) the selection of pre-trained models, including image classifiers and text-image encoders; and 3) model output mapping strategies, including nonparametric and trainable label mapping. Our extensive experimental results show that AutoVP outperforms the best-known current VP methods by a substantial margin, having up to 6.7% improvement in accuracy; and attains a maximum performance increase of 27.5% compared to linear-probing (LP) baseline. AutoVP thus makes a two-fold contribution: serving both as an efficient tool for hyperparameter tuning on VP design choices, and as a comprehensive benchmark that can reasonably be expected to accelerate VP's development. The source code is available at https://github.com/IBM/AutoVP.

==> assets/tables/detection_acc.tex <==
\begin{table}[h] 
\caption{\textbf{Performance on Detection Datasets.} The IoU scores of linear probing (LP) and AutoVP.}  \label{tab:detect_acc}
\centering
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{c|c|c|c}
\hline
Dataset & Zero-shot   & Finetune box head & VP          \\ \hline
VOC     & IoU: 0.7588 & IoU: \textbf{0.7629}       & IoU: 0.7371 \\ \hline
ISIC    & IoU: 0.5246 & IoU: 0.7081       & IoU: \textbf{0.8055} \\ \hline
\end{tabular}
\end{table}

==> assets/tables/model_comparision.tex <==
% https://www.tablesgenerator.com/
\begin{table}[h]
\caption{\textbf{Pre-Trained Model Comparision.} The testing accuracy (\%) on 12 datasets was evaluated using the four pre-trained classifiers within the AutoVP framework. The highest accuracy across pre-trained models is indicated in \textbf{bold}.}
\label{Rebuttal:model_comparision}
\centering
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{c|c|c|c|c}
\hline
Datasets   & ResNet18 & ResNeXt101-IG  & Swin-T         & CLIP          \\ \hline
SVHN       & 83.7    & 85.6          & 90.7          & \textbf{92.9} \\ \hline
CIFAR10    & 87.8    & \textbf{95.9} & 93.3          & 95.2          \\ \hline
Flowers102 & 85.4    & 92.2          & \textbf{93.5} & 90.4          \\ \hline
Food101    & 54.2    & 80.6          & 75.9          & \textbf{82.3} \\ \hline
UCF101     & 55.9    & 71.6          & 73.0          & \textbf{73.1} \\ \hline
OxfordIIITPet       & 82.7    & \textbf{94.2} & 90.2          & 88.2          \\ \hline
CIFAR100   & 63.7    & \textbf{79.8} & 76.5          & 77.9          \\ \hline
EuroSAT    & 93.0    & 94.0          & 96.0          & \textbf{96.8} \\ \hline
DTD        & 54.8    & \textbf{69.5} & 69.3          & 62.5          \\ \hline
ISIC       & 67.4    & 67.4          & 71.7          & \textbf{74.0} \\ \hline
FMoW       & 30.2    & 32.5          & 39.8          & \textbf{40.8} \\ \hline
GTSRB      & 81.5    & 80.0          & 88.1           & \textbf{93.1} \\ \hline
Average    & 70.0    & 78.6          & 79.8          & \textbf{80.6} \\ \hline
\end{tabular}
\vspace{-4mm}
\end{table}

==> assets/tables/other_ds.tex <==
\begin{table}[h]
\caption{\textbf{Performance on Additional Datasets.} The testing accuracy (\%) for four additional datasets commonly found in VP research.}
\label{ICLR_Rebuttal:other_dataset}
\centering
\renewcommand{\arraystretch}{1.5}
\scalebox{1}{
\begin{tabular}{c|c|c|c|c|c}
\hline
Dataset     & AutoVP Setting  & AutoVP        & LP   & ILM           & CLIP-VP \\ \hline
SUN397      & FullyMap, p=16  & \textbf{65.4} & 70.9 & 61.2          & 60.5    \\ \hline
StanfordCar & FullyMap, p=16  & \textbf{61.8} & 77.6 & 57.6          & 56.2    \\ \hline
RESISC      & FullyMap, p=17  & \textbf{88.5} & 91.7 & 86.6          & 84.5    \\ \hline
CLEVR       & FullyMap,  p=16 & 83.0          & 68.0 & \textbf{83.1} & 81.4    \\ \hline
\end{tabular}
}
\end{table}
